Computer modelling of accretion processes in binary systems with black holes and neutron stars

This dissertation is written as an annotated collection of selected articles. The dissertation focuses on the modelling of accretion disks in X-ray binaries with a black hole or neutron star. The main objective is to use advanced numerical methods to reveal the fundamental processes that influence the observed spectral and temporal features. Among the significant results of this modelling is the recognition of the puffy accretion disk, a novel type of accretion disk based purely on the results of numerical simulations. Furthermore, the work focuses on modelling the X-ray variability and quasi-periodic oscillations using analytical models of accretion disks, but an advanced description of the oscillations, and a discussion of the implications of this modelling for observational data.

==> babelbst.tex <==
%% $Id: babelbst.tex,v 0.3 2007/02/23 09:35:47 sta Exp $
%% The structure of this file depends on your language selection
%% in the `latex' and/or `pdflatex' format.  This can be achieved
%% by inspecting language file `language.dat' (typically location
%% is /var/lib/texmf/tex/generic/config/language.dat, but this
%% can vary from distro to distro).  Follow instruction in this
%% file and activate the languages required (US-English should
%% always be activated as the first, i.e., number 0 language).
%% Then re-generate the above formats.  The selected languages
%% are numbered starting from 0 (American English).  Check the
%% language enumeration by inspecting the format generation log
%% files latex.log and/or pdflatex.log (search for the string
%% \language).  Now, in the switch structure below, input
%% bibliography language definition (.bld) file belonging to
%% the language number as described above in the corresponding
%% branch of the `\ifcase' switch structure.  If required, feel
%% free to add further languages.  Good luck.
%%

\ifcase\language % 0=american(=USenglish)
  \input{american.bld}
\or % 1=british(=UKenglish=english)
  \input{british.bld}
\or % 2=french(=patois)
  \input{french.bld}
\or % 3=german(=austrian)
  \input{german.bld}
\or % 4=ngerman(=naustrian)
  \input{ngerman.bld}
\or % 5=czech
  \input{czech.bld}
\or % 6=slovak
  \input{slovak.bld}
\else % 7=nohyphenation
  \input{american.bld}
\fi




\endinput
%%
%% End of file `babelbst.tex'.


==> staff.tex <==
%%
%% $Id: staff.tex,v 0.13 2011/12/10 19:17:47 lvs Exp $
%%
%% Soubor se jmény vyučujících ÚF a částečně i ÚMI a jiných pracovišť
%% Revize:
%% 30.10.1996 S.H.
%% 31. 1.1997 S.H. (aktualizace)
%% 20. 5.1999 ---sh (aktualizace)
%% 14.10.1999 ---sh (odstraněna ostudná chyba s proděkankou Pískovou)
%% 18.10.1999 ---sh (doplněn \techedit)
%% 16. 2.2000 ---sh (doplněna Mgr. Jedličková)
%% 24. 7.2000 ---sh (změna proděkana)
%% 12.11.2000 ---sh (úprava titulu)
%%  3. 1.2002 ---sh (Zdeněk profesor)
%% 11. 5.2002 ---sh (dopl.sekr. I. Bryjová, P. Slaný, J. Juráň; Běták docentem)
%% 17. 5.2002 ---sh (opravena Jedličková)
%% 21. 5.2002 ---sh (opět opravena na Mgr. Jedličková)
%%  8. 8.2002 ---sh (Hynek Sekanina Ph.D.)
%% 27. 5.2003 ---sh (nástup Ing. J. Zemana)
%% 15. 3.2004 ---sh (doplněn Marek Abramowicz)
%%  6. 9.2004 ---sh (doplněni aktuální doktorandi)
%%  5. 5.2005 ---sh (doplněni Cip, Bak, Cer, Kuc)
%% 14.10.2005 ---sh (Kamilino nové příjmení)
%%  8. 1.2006 ---sh (údržba)
%%  3.10.2006 ---sh (údržba: Bc. Bakala -> Mgr. Bakala)
%%  5.10.2006 ---sh (údržba: Mgr. -> RNDr. Török, Juráň, Kovář, Slaný;
%%                  přidána Šrámková)
%% 11.12.2006 ---sh (přidán Petr Čermák)
%% 11.10.2007 ---sh (Bc. Ivety, přidáni další členové a doktorandi ÚF)
%% 17. 2.2009 ---sh (údržba: Mgr. Bakala -> RNDr. Bakala)
%% 20. 2.2009 ---sh (přidán T. Gráf)
%% 30.10.2009 ---sh (přidán Mgr. K. Adámek, Mgr. J. Novotný)
%% 12. 9.2010 ---sh (aktualizace při stěhování do `code')
%% 29.11.2010 ---sh (přidán Mgr. Petr Čech)
%%  5. 9.2011 ---sh (oprava CecP -> cecp, Prof., Doc. s verzálkou)
%% 14.12.2014 ---sh (Hledík: přidán doc., prof. doc. s minuskulí)
%%

%% Tituly %%
\def\ing{Ing.}
\def\prof{prof.}
\def\doc{doc.}

%% ÚF %%
\def\Stu{\prof~RNDr.~Zdeněk~Stuchlík,~CSc.}
\def\stu{\prof~Z.~Stuchlík}
\def\Abr{\prof~Marek Abramowicz}
\def\abr{\prof~M.~Abramowicz}
\def\Lic{\prof~\ing~Peter~Lichard,~DrSc.}
\def\lic{\prof~P.~Lichard}
\def\Hub{\prof~PhD~Ivan~Hubač,~DrSc.}
\def\hub{\prof~I.~Hubač}
\def\Cer{\prof~RNDr.~Martin~Černohorský,~CSc.}
\def\cer{\prof~M.~Černohorský}
\def\Hab{\doc~\ing~Petr~Habrman,~CSc.}
\def\hab{\doc~P.~Habrman}
\def\Pis{\prof~\ing~Jaromír~Pištora,~CSc.}
\def\pis{\prof~J.~Pištora}
\def\Bet{\doc~RNDr.~Emil~Běták,~DrSc.}
\def\bet{\doc~Dr.~E.~Běták}
\def\Hlu{\doc~RNDr.~Petr~Hlubina,~CSc.}
\def\hlu{\doc~P.~Hlubina}
\def\Hle{\doc~RNDr.~Stanislav~Hledík,~Ph.D.}
\def\hle{\doc~S.~Hledík}
\def\Sek{RNDr.~Hynek~Sekanina,~Ph.D.}
\def\sek{Dr.~H.~Sekanina}
\def\Sla{RNDr.~Petr~Slaný,~Ph.D.}
\def\sla{Dr.~P.~Slaný}
\def\Jur{RNDr.~Josef~Juráň,~Ph.D.}
\def\jur{Dr.~J.~Juráň}
\def\JanT{\ing~Tomáš~Janečka}
\def\janT{\ing~T.~Janečka}
\def\Sva{Mgr.~Richard~Švacha}
\def\sva{Mgr.~R.~Švacha}
\def\Val{\ing~Miroslav~Vala,~CSc.}
\def\val{\ing~M.~Vala}
\def\Zem{Bc.\,\&\,BcA.~Miroslav~Zeman}
\def\zem{Bc.~M.~Zeman}
\def\ZemJ{\ing~Jaroslav~Zeman}
\def\zemJ{\ing~J.~Zeman}
\def\Tor{RNDr.~Gabriel Török,~Ph.D.}
\def\tor{Dr.~G. Török}
\def\Mra{Mgr.~Kristina Mrázová}
\def\mra{Mgr.~K. Mrázová}
\def\Pls{Mgr.~Kamila Truparová Plšková}
\def\pls{Mgr.~K. Truparová Plšková}
\def\Urb{Mgr.~Martin Urbanec,~Ph.D.}
\def\urb{Dr.~M. Urbanec}
\def\Hor{Mgr.~Petr Horsák}
\def\hor{Mgr.~P. Horsák}
\def\Hla{Mgr.~Jan Hladík}
\def\hla{Mgr.~J. Hladík}
\def\Hlav{Bc.~Aleš Hlaváček}
\def\hlav{Bc~A. Hlaváček}
\def\Kov{RNDr.~Jiří Kovář,~Ph.D.}
\def\kov{Dr.~J. Kovář}
\def\Cip{Mgr.~Alois Cipko}
\def\cip{Mgr.~A. Cipko}
\def\Bak{RNDr.~Pavel Bakala,~Ph.D.}
\def\bak{Dr.~P. Bakala}
\def\Cer{Mgr.~Slavomír Černý}
\def\cer{Mgr.~S. Černý}
\def\Pet{Mgr.~Martin Petrásek}
\def\pet{Mgr.~M. Petrásek}
\def\CerP{\doc~\ing~Petr~Čermák,~Ph.D.}
\def\cerp{\doc~P.~Čermák}
\def\Kuc{Mgr.~Hana Kučáková}
\def\kuc{Mgr.~H. Kučáková}
\def\Kot{Mgr. \ing~Andrea Kotrlová,~Ph.D.}
\def\kot{Dr.~A. Kotrlová}
\def\Sche{Mgr.~Jan Schee,~Ph.D.}
\def\sche{Dr.~J. Schee}
\def\Gra{RNDr.~Tomáš Gráf,~Ph.D.}
\def\gra{Dr.~T. Gráf}
\def\Uhl{Mgr. Milan Uhlár, Ph.D.}
\def\uhl{Dr. M. Uhlár}
\def\Voj{Mgr.~Martin Vojík,~Ph.D.}
\def\voj{Dr.~M. Vojík}
\def\Kol{Mgr.~Martin Kološ}
\def\kol{Mgr.~M. Kološ}
\def\Sra{RNDr.~Eva Šrámková,~Ph.D.}
\def\sra{Dr.~E. Šrámková}
\def\NovJ{Mgr.~Jan Novotný}
\def\novj{Mgr.~J. Novotný}
\def\AdaK{Mgr.~Karel Adámek}
\def\adak{Mgr.~K. Adámek}
\def\CecP{Mgr.~Petr Čech}
\def\cecp{Mgr.~P. Čech}
\def\Bry{Ing.~Iveta Bryjová}
\let\bry\Bry
%\def\BAr{Vojtěch~Bartek,~ASČF}
%\def\Bar{Vojtěch~Bartek}
%\def\bar{V.~Bartek}
\def\vicedean{PhDr.~Irena~Korbelářová,~Dr.}
\def\techedit{Dana Panajotidisová}

\endinput

%%
%% End of file `staff.tex'.

